Integral monodromy groups of Kloosterman sheaves

We show that integral monodromy groups of Kloosterman $\ell$-adic sheaves of rank $n\ge 2$ on $\mathbb{G}_m/\mathbb{F}_q$ are as large as possible when the characteristic $\ell$ is large enough, depending only on the rank. This variant of Katz's results over $\mathbb{C}$ was known by works of Gabber, Larsen, Nori and Hall under restrictions such as $\ell$ large enough depending on $\operatorname{char}(\mathbb{F}_q)$ with an ineffective constant, which is unsuitable for applications. We use the theory of finite groups of Lie type to extend Katz's ideas, in particular the classification of maximal subgroups of Aschbacher and Kleidman-Liebeck. These results will apply to study reductions of hyper-Kloosterman sums in forthcoming work.

==> commands.tex <==
%auto-ignore

\newcommand{\declarecommand}[1]{\providecommand{#1}{}\renewcommand{#1}}

% Miscellaneous
\newcommand{\cdotarg}{\, \cdot \,}
\newcommand{\co}{\backslash}
\newcommand{\normal}{\mathrel{\unlhd}}
\newcommand{\dia}[1]{\langle#1\rangle}
\newcommand{\mtu}{\,--\,}
\newcommand{\closure}{\overline}
\newcommand*\elide{\textup{[\,\dots]}}
\newcommand{\sump}{\sideset{}{'}\sum}

%Floor/Ceil
\providecommand{\ceil}[1]{\left \lceil #1 \right \rceil }
\providecommand{\floor}[1]{\left \lfloor #1 \right \rfloor }

%Matrix groups and Lie algebras
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\GU}{\operatorname{GU}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\SL}{\operatorname{SL}}
\declarecommand{\sl}{\mathfrak{sl}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spin}{\operatorname{Spin}}
\newcommand{\so}{\mathfrak{so}}
\declarecommand{\O}{\operatorname{O}}
\newcommand{\GO}{\operatorname{GO}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\GSp}{\operatorname{GSp}}
\declarecommand{\sp}{\mathfrak{sp}}
\newcommand{\PSp}{\operatorname{PSp}}
\newcommand{\PSO}{\operatorname{PSO}}
\newcommand{\USp}{\operatorname{USp}}
\newcommand{\PSU}{\operatorname{PSU}}

% Blackboard
\newcommand{\A}{\mathbb{A}}
\declarecommand{\P}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\HI}{\mathbb{H}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}

% Kloosterman
\newcommand{\Kl}{\operatorname{Kl}}
\newcommand{\Klc}{\mathcal{K}l}

% Operators
\declarecommand{\Hom}{\operatorname{Hom}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\arctanh}{\operatorname{arctanh}}
\newcommand{\Inn}{\operatorname{Inn}}
\newcommand{\Out}{\operatorname{Out}}
\newcommand{\Graph}{\operatorname{Graph}}
\newcommand{\genus}{\operatorname{genus}}
\newcommand{\Jac}{\operatorname{Jac}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Li}{\operatorname{Li}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\cond}{\operatorname{cond}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sing}{\operatorname{Sing}}
\newcommand{\Swan}{\operatorname{Swan}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\Isom}{\operatorname{Isom}}
\newcommand{\Lie}{\operatorname{Lie}}
\newcommand{\dropp}{\operatorname{drop}}
\newcommand{\trdeg}{\operatorname{trdeg}}
\newcommand{\der}{\mathrm{der}}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\height}{\operatorname{height}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\car}{\operatorname{char}}
\newcommand{\charpol}{\operatorname{charpol}}
\newcommand{\inv}{^{-1}}
\newcommand{\disc}{\operatorname{disc}}
\newcommand{\lspan}{\operatorname{span }}
\newcommand{\fix}{\operatorname{fix}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Fr}{\operatorname{Fr}}
\newcommand{\ch}{\operatorname{ch}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Symm}{\operatorname{Symm}}
\newcommand{\Twists}{\operatorname{Twists}}
\newcommand{\Alt}{\operatorname{Alt}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Div}{\operatorname{Div}}
\declarecommand{\Re}{\operatorname{Re}}
\newcommand{\res}{\operatorname{res}}
\declarecommand{\Im}{\operatorname{Im}}
\declarecommand{\Spec}{\operatorname{Spec}}
\declarecommand{\Proj}{\operatorname{Proj}}
\newcommand{\rank}{\operatorname{rank}}
\declarecommand{\supp}{\operatorname{supp}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\FT}{\operatorname{FT}}
\newcommand{\mult}{\operatorname{mult}}
\newcommand{\orb}{\operatorname{orb}}
\newcommand{\Std}{\operatorname{Std}}
\newcommand{\Cov}{\operatorname{Cov}}
\declarecommand{\Var}{\operatorname{Var}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}

\newcommand{\No}{\operatorname{N}} % Normalizer
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\hol}{\mathrm{hol}}
\newcommand{\alg}{\mathrm{alg}}
\declarecommand{\div}{\mathrm{div}}
\declarecommand{\pdiv}{\mathrm{pdiv}}
\newcommand{\prob}{\mathrm{prob}}
\newcommand{\geom}{\mathrm{geom}}
\declarecommand{\ss}{\mathrm{ss}}
\newcommand{\arith}{\mathrm{arith}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\old}{\mathrm{old}}

% Fraktur
\newcommand{\af}{\mathfrak{a}}
%\declarecommand{\bf}{\mathfrak{b}}
\newcommand{\cf}{\mathfrak{c}}
\newcommand{\gf}{\mathfrak{g}}
\newcommand{\pf}{\mathfrak{p}}
\newcommand{\qf}{\mathfrak{q}}
\newcommand{\lf}{\mathfrak{l}}
\newcommand{\Pf}{\mathfrak{P}}
\newcommand{\mf}{\mathfrak{m}}
\newcommand{\Mf}{\mathfrak{M}}
\newcommand{\Sf}{\mathfrak{S}}

% Cal
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\declarecommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Cl}{\mathcal{C}l}


%Legendre symbol
\newcommand{\legendre}[2]{\left(\frac{#1}{#2}\right)}
\newcommand{\dlegendre}[2]{\left(\frac{#1}{#2}\right)}

%Bold symbols and letters
\declarecommand{\bs}{\boldsymbol}
\newcommand{\Gb}{\bm{G}}
\newcommand{\Tb}{\bm{T}}
\newcommand{\Vb}{\bm{V}}

% Averages
\newcommand{\aver}[3]{\frac{1}{#3}\sum_{#1\in #2}}
\newcommand{\averC}[2]{\aver{#1}{#2}{|#2|}}

%TODO
\newcommand{\TODO}[1]{[{\color{red}\sffamily\textbf{todo:} #1}]}
\newcommand{\later}[1]{[{\color{black}\sffamily\small\textbf{later:} #1}]}
\newenvironment{TODOb}{\color{red}\sffamily{\begin{center}\rule{0.4\textwidth}{0.5pt}\textbf{TODO}\rule{0.4\textwidth}{0.5pt}\end{center}}}{\begin{center}\rule{\textwidth}{0.5pt}\end{center}}
%\definecolor{light-gray}{gray}{0.5}
%\newenvironment{remove}{\color{light-gray}\sffamily}{}

%http://tex.stackexchange.com/questions/58141/equations-inside-enumerate-aligned-on-items-number
\newcommand\Item[1][]{%
  \ifx\relax#1\relax  \item \else \item[#1] \fi
  \abovedisplayskip=0pt\abovedisplayshortskip=0pt~\vspace*{-\baselineskip}}

%https://tex.stackexchange.com/questions/39221/removing-extra-space-with-pmod-command
\makeatletter
\let\@@pmod\pmod
\DeclareRobustCommand{\pmod}{\@ifstar\@pmods\@@pmod}
\def\@pmods#1{\mkern4mu({\operator@font mod}\mkern 6mu#1)}
\makeatother

%http://tex.stackexchange.com/questions/4302/prettiest-way-to-typeset-c-cplusplus
\newcommand{\CC}{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\tiny\bf +}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\tiny\bf +}}
\def\CC{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\tiny\bf ++}}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand{\mailto}[1]{\href{mailto:#1}{#1}}

%https://tex.stackexchange.com/questions/169907/how-to-typeset-the-house-of-an-algebraic-number
\makeatletter
\newcommand*{\house}[1]{%
  \mathord{%
    \mathpalette\@house{#1}%
  }%
}
\newcommand*{\@house}[2]{%
  % #1: math style
  % #2: expression that gets the "house"
  % get the line width of `\overline' in the current math font size
  \dimen@=\fontdimen8 %
      \ifx#1\scriptscriptstyle\scriptscriptfont
      \else\ifx#1\scriptstyle\scriptfont
      \else\textfont\fi\fi
      3 %
  \sbox0{%
    $#1%
      \vrule width\dimen@\relax
      \overline{%
        \kern2\dimen@
        \begingroup % to keep changes of \dimen@ in #2 local
          #2%
        \endgroup
        \kern2\dimen@
      }%
      \vrule width\dimen@\relax
      \mathsurround=1.5\dimen@ % outside margin
    $%
  }%
  % TeX adds an empty space above `\overline', it needs to be
  % removed to get the correct height for the `\vrule's
  \ht0=\dimexpr\ht0-\dimen@\relax
  \dp0=\dimexpr\dp0+2\dimen@\relax
  \vbox{%
    \kern\dimen@ % reinsert previously removed space
    \copy0 %
  }%
}

==> enumerate.tex <==
%auto-ignore
\renewcommand{\labelitemi}{--}

\usepackage[inline,shortlabels]{enumitem} % Call after babel
%\setenumerate{itemsep=0mm,topsep=0.1cm}
\setenumerate[1]{label={(\arabic*)}}

==> hyperref.tex <==
%auto-ignore
\usepackage[lowtilde]{url}
\usepackage[linktocpage,bookmarksdepth=2]{hyperref}
\hypersetup{
%    hidelinks,
     colorlinks,
     linkcolor=green,
     citecolor=green,
     urlcolor=blue
}
\urlstyle{rm}

==> packages.tex <==
%auto-ignore
\usepackage{etex}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathabx}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{graphicx}
%\usepackage{grffile}
\usepackage{pstricks}
\usepackage{pst-plot}
\usepackage{pstricks-add}
\usepackage{bm}
\usepackage{fp}
\usepackage{multido}
\usepackage{subfig} %conflicts with tocloft
\psset{algebraic=true}
\usepackage[all]{xy}
\usepackage{subfiles}
\usepackage{multicol}

\usepackage{color}
\definecolor{vlightgray}{gray}{0.95}

%Adjust bibliography spacing and font size
% \makeatletter
% \@ifclassloaded{amsart}
% {

% %For arxiv submissions
\let\OLDthebibliography\thebibliography
\renewcommand\thebibliography[1]{
\OLDthebibliography{#1}
\setlength{\parskip}{0pt}
\setlength{\itemsep}{0.3cm}
}
\renewcommand{\bibliofont}{\small}
% }
% {

%\usepackage{natbib}
%\setlength{\bibsep}{0.3cm}
%\def\bibfont{\small}

%} 
%\makeatother
%With biblatex
%\usepackage[style=trad-alpha]{biblatex}
%\renewcommand*{\bibfont}{\small}
%\setlength\bibitemsep{0.3cm}
%With bibtex

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

==> theorems.tex <==
%auto-ignore
\newcounter{theoscounter}
%\numberwithin{theoscounter}{section}
\newtheoremstyle{thm}{0.4cm}{0.4cm}{\itshape}{}{\bfseries}{.}{.5em}{}
\newtheoremstyle{def}{0.3cm}{0.3cm}{}{}{\scshape}{.}{.5em}{}
\newtheoremstyle{exre}{0.4cm}{0.4cm}{}{}{\itshape}{.}{.5em}{}

\theoremstyle{def}
\let\definition\relax
\newtheorem{definition}[theoscounter]{Definition}
\newtheorem{notation}[theoscounter]{Notation}
\newtheorem{convention}[theoscounter]{Convention}

\theoremstyle{thm}
\newtheorem{theorem}[theoscounter]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theoscounter]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{corollary}[theoscounter]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{claim}[theoscounter]{Claim}
\newtheorem{lemma}[theoscounter]{Lemma}
\newtheorem*{lemma*}{Lemma}

\theoremstyle{exre}
\newtheorem{conjecture}[theoscounter]{Conjecture}
\newtheorem{question}[theoscounter]{Question}
\newtheorem*{question*}{Question}
\newtheorem{example}[theoscounter]{Example}
\newtheorem*{example*}{Example}
\newtheorem{examples}[theoscounter]{Examples}
\newtheorem*{examples*}{Examples}
\newtheorem{questions}[theoscounter]{Questions}
\newtheorem{remark}[theoscounter]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem*{acknowledgements}{Acknowledgements}
\newtheorem{remarks}[theoscounter]{Remarks}
\newtheorem*{remarks*}{Remarks}

%\numberwithin{theoscounter}{section}

